Internal Feedback in Biological Control: Diversity, Delays, and Standard Theory

Neural architectures in organisms support efficient and robust control that is beyond the capability of engineered architectures. Unraveling the function of such architectures is challenging; their components are highly diverse and heterogeneous in their morphology, physiology, and biochemistry, and often obey severe speed-accuracy tradeoffs; they also contain many cryptic internal feedback pathways (IFPs). We claim that IFPs are crucial architectural features that strategically combine highly diverse components to give rise to optimal performance. We demonstrate this in a case study, and additionally describe how sensing and actuation delays in standard control (state feedback, full control, output feedback) give rise to independent and separable sources of IFPs. Our case study is an LQR problem with two types of sensors, one fast but sparse and one dense but slow. Controllers using only one type of sensor perform poorly, often failing even to stabilize; controllers using both types of sensors perform extremely well, demonstrating a strong diversity-enabled sweet spot (DESS). We demonstrate that IFPs are key in enabling this DESS, and additionally that with IFPs removed, controllers with delayed sensing perform poorly. The existence of strong DESS and IFP in this simple example suggest that these are fundamental architectural features in any complex system with diverse components, such as organisms and cyberphysical systems.

==> unused/old_background.tex <==
\section{Background \& Motivation} \label{sec:Background}

\subsection{Key concepts}
Fig. \ref{fig:intro_figure_neuro} demonstrates some examples of the enormous amount of IFPs present in brains. However, it is also a simplified figure that hides the enormous complexity of the underlying cells, neurons, and networks. We introduce four key concepts necessary to begin to untangle this complexity.

\subsubsection{Levels} The most familiar concept is that biology has distinct \textit{levels}, or scales (e.g. from molecules to synapses, cells, and circuits). Fig. \ref{fig:intro_figure_neuro} hides lower level implementations in neural hardware. 

\subsubsection{Speed-accuracy tradeoffs (SATs)} Biological hardware has severe speed-accuracy tradeoffs (SATs), a familiar concept that is expanded and extended in our theory and experiments. SATs are prevalent at the hardware level, but less so at the behavioral level.

\subsubsection{Diversity-enabled sweet spots (DESS)} Introduced in \cite{Nakahira2021}. Highly diverse hardware-level components (which obey SATs) enable performance sweet-spots which overcome the hardware-level SATs. Extreme diversity in axon sizes, receptors, and neurotransmitters are abundant but largely hidden in Fig. \ref{fig:intro_figure_neuro}. By itself, diversity of components only enables sweet spots; to achieve these sweet spots requires specific architectures to maximize the utility of each component. We present a numerical example in Section \ref{sec:DESS}.

\subsubsection{Layered architecture} Layered architecture (e.g. reflex layer vs. planning layer) helps create DESS \cite{Nakahira2021}. We claim that DESS is universal, but architecture remains an ad hoc and domain-specific subject, something we aim to change.

Fig. \ref{fig:intro_figure_sls}a highlights the essential concepts of layered architecture, SATs, and DESS but with the simplest possible experiments and theory \cite{Liu2019, Nakahira2021}. Naively, success seems to require speed and accuracy that this hardware lacks, making non-layered solutions infeasible. Our layered brain breaks the overall problem into a high ``trails'' layer of slow but accurate vision with trail look-ahead for advanced warning, and a low ``bumps'' layer that uses fast but inaccurate muscle spindles and proprioception to sense and reject bump disturbances. Their motor commands to the muscles simply add. The resulting layers multiplex well in experiments and theory. Effective architectures (e.g. layering) creates a DESS where diverse hardware enables a sweet spot that is both fast and accurate despite having no hardware that is. Across a wide range of conditions, theory and data agree, and all are remarkably robust to assumptions and details (e.g worst-case vs. stochastic). All experiments and theory require only high-school level math, and the formulas for optimal controllers and the resulting errors are analytic, simple, and transparent. 

\subsection{SATs, diversity, and IFPs in biology}
The primate sensorimotor system uses components with SATs and diversity in response speeds. We can divide the sensorimotor system into a fast layer (i.e. proprioception, the ability to sense position movements of our body) and a slow layer (i.e. visual cortex), as is done in \cite{Nakahira2021}. Proprioceptive reaction time is $95.6 \pm 10.6$ ms \cite{Manning2012}, while visual reaction time is much slower at $247.6 \pm 18.54$ ms \cite{Jain2015}. Proprioception is fast but inaccurate; when performing sensorimotor tasks, we rely on vision for precision and accuracy \cite{Sarlegna2009}. On the motor side, we also possess diverse muscle fibers that obey SATs; inaccurate fast-twitch muscles, and accurate slow-twitch muscles. Though the diverse components of the sensorimotor system obey SATs, they are combined in a layered architecture that enables performance that is both fast and accurate, i.e. a DESS in performance \cite{Nakahira2021}.

The immune system response also contains diverse parts obeying SATs. The immune system can roughly be divided into two parts: innate and adaptive immunity. Innate immunity provides fast, somewhat inaccurate protection, and can limit infections. Cells such as macrophages, neutrophils and basophils respond rapidly, within minutes to hours. Adaptive immunity is accurate but slow, providing specialized protection against pathogens. Adaptive immune responses can take up to weeks, but are very effective; T lymphocytes and B lymphocytes work to produce efficient and long lasting protection. As in the sensorimotor system, the diverse components of the immune system are combined in biological architecture that give a DESS in speed and accuracy.

Within vision, IFPs are abundant and well-documented \cite{Felleman1991, CALLAWAY2004, MUCKLI2013}. This is also shown in Fig. \ref{fig:intro_figure_neuro}a, and discussed at length in previous sections. IFPs are also present in the immune system, where T cells can be further divided into CD4+ T cells, i.e. T helper and regulatory cells, and CD8+ T cells, i.e. cytotoxic T cells. While CD8+ T cells can be thought of as actuators in the control sense, helper and regulatory cells mediate much more complicated dynamics that suppress or amplify CD8+ cells as well as innate immune sensory circuits \cite{Busse2010,Lund2008,Palm2007}. Collectively, these elements suggest that IFPs are abundantly present in the immune system in order to recognize and be sensitive to changes and irregularities.

\subsection{Architectures in controllers}
To explain the ubiquity of IFPs and integrate the above concepts, we use theory from standard control and SLS.

Biological control uses components (i.e. cells, neurons) that are sparse, local, delayed, saturating, noisy, and distributed. We shall refer to these as \textit{SLD+ constraints}; they are essential for producing realistic models. The inclusion of such constraints allow us to model diverse components and the resultant DESS. However, existing theories from optimal and robust control become computationally intractable even with minimal combinations of SLD+ constraints. In contrast, SLS explicitly allows for the inclusion of SLD+ constraints on sensing, communication, and actuation. This allows us to model SATs at various levels of biology. SLS not only produces optimal controllers under SLD+ constraints, but also yields novel controller architectures containing striking similarities (i.e. abundant IFPs) to biological architectures \cite{Paper2}. This inspired us to return to standard, ``pre-SLS'' controllers and dig deeper into their architecture, which were generally unexamined. We focus on pre-SLS controllers with delayed sensing in Sections \ref{sec:DESS} and \ref{sec:IFP}, and discuss what such controllers can tell us about IFP and architecture.

SLS and SLD+ constraints are complementary to the notions of DESS and layered architecture; a full model of biological control includes both, as suggested in Fig. \ref{fig:intro_figure_sls}. Though Fig. \ref{fig:intro_figure_sls}a describes important concepts, it abstracts away underlying architectural details such as massive amounts of IFPs. Boxes and wires in this figure are, as in Fig. \ref{fig:intro_figure_neuro}, schematic drawings of systems whose lower levels are implemented in hardware level neurons, sensors, muscles, all of which obey SATs and SLD+ constraints. To expand the model and uncover the underlying IFPs, SLS is required.

Fig. \ref{fig:intro_figure_sls}b expands the green reflex box from \ref{fig:intro_figure_sls}a. Here, we sense the full state with delay, creating IFPs in the optimal controller. This is explored in a more concrete example in Section \ref{sec:IFP}. This figure presents a simple case in which rich IFPs arises from a single, neurally plausible mechanism: sensing delay. An orthogonal direction in Fig \ref{fig:intro_figure_sls}c imposes local communication constraints (i.e. locality) on the internal communications and computing hardware. The result is an explosion in the amount of IFPs and internal memory that is difficult to visualize even in the simplest case; we refer the reader to \cite{Paper2} for more detailed visualizations. This figure demonstrates another simple case wherein rich IFP arises from a single, neurally plausible mechanism: this time, local communication. We emphasize that SLS is able to accommodate delay and locality constraints easily. 

IFPs arising from both delay and locality can be loosely interpreted as predictive; they are dominated by the known effects of our actions and how they propagate through the plant dynamics, which include the body and its environment. They also depend on what the objective of our future actions are, and most importantly how communication delays limit such actions. This is much more than Bayesian prediction, which is pedagogically important given its popularity, but is a very special and ultimately minor source of IFP in reality; we briefly discuss this in Section \ref{sec:IFP}. Our view of IFP is consistent with recent experiments \cite{Musall2019, Stringer2019}.

In addition to locality and delay constraints, there are other realistic constraints beyond those in Fig. \ref{fig:intro_figure_sls} (e.g. actuator saturation) that cause further increases in the amount of IFPs. These constraints are nevertheless entirely comprehensible with SLS. Superficially, the SLS ``physiology'' of Fig. \ref{fig:intro_figure_sls}b-c has many of the features of Fig. \ref{fig:intro_figure_neuro}; we anticipate that incorporating additional constraints will strengthen the similarity.

The above theory is not only essential to biological architectures but to engineering architectures as well. Fast electronic components allow us to avoid most SLD+ constraints in current engineered systems; however, these components are much less energy-efficient than their biological counterparts. As we move toward sustainable, energy-efficient infrastructures and large networked systems (e.g. smart grids), SLD+ constraints will become unavoidable. A cohesive theory of DESS and architecture will allow engineers to fully exploit the full range of engineering components to create the best possible performance for these future systems.


==> unused/old_conclusion.tex <==
\subsection{Experimental Predictions}
By computing optimal controllers (via SLS) with SLD+ constraints, we can design increasingly complicated architectures for which we can precisely explain the function of each component. These optimal controllers may not perfectly match neurobiology, but will lead to more refined experimental directions. Distinct from traditional models, our controller models produce \textit{a priori} models of architecture and behavior from experimentally determined constraints (e.g. delays) as in Fig. \ref{fig:intro_figure_sls}. Our models allow us to make comparisons with all layers and levels of experimental data in a way that conventional models do not; this will make connections between levels, layers, and behavior more transparent. Below, we propose concrete experiments\footnote{Though theoretical concepts discussed in this paper apply to general organisms, biological experiments necessarily require engagement with details of a specific model system.}.

Neuronal circuits for escape behaviors in the fruit fly \textit{Drosophila melanogaster} have long been important models for unraveling neural control of behavior because they contain experimentally tractable large axons specialized for rapid conduction, and hard-wired dedicated circuits with few synapses from sensor to motor that drive critical escape actions \cite{Carew1985}. This has led to a model that behavior is controlled by dedicated FFPs \cite{kristan2008}. This view is too simple, as such a system could not be robust to the wide range of attack scenarios that real animals encounter. Recently, dynamical frameworks have been applied to complex behaviors, e.g. replacing processing in individual neurons with attractor states of neural population activity \cite{kristan2008, Wang2002}. However, what is still missing from our current biological understanding is how nervous systems make flexible decisions at the component level, and in particular, how IFPs (not just FFPs) from different parts of the nervous system may be integrated to achieve behavioral goals. We expect that the theory described in this paper and its companion \cite{Paper2} will help to surmount these current gaps in understanding of action generation and selection during naturally-occurring behaviors.

Adult flies contain a unique descending neuron specialized for rapid conduction: the large-axon Giant Fiber (GF). The GF integrates photoreceptor information and projects to the nerve cord, where it synapses directly on the motor neuron that drives the ``jump" muscle. The timing of a single spike in the GF determines whether the fly will choose speed (fast takeoff) or accuracy (slow takeoff) in its escape \cite{vonReyn2017, Ache2019_looming, vonReyn2014}. The GF comprises a strong FFP from photoreceptor to muscle, for which we know identity of each neuron and, at least conceptually, the computation performed across each synapse. This pathway participates in a multi-layered visual processing system in which component diversity (axon diameter) is a prominent feature. The theory described above and in \cite{Paper2} offers an initial theoretical explanation not only for what the GF system should do but for what information must be carried by IFPs to the dendrites of the the Giant Fiber in order to make rapid responses possible. In larvae, this leads to the more speculative prediction that previously unidentified feedback circuits mediate escape behaviors.

Central to our goal of uniting biological mechanisms with structured control components is our ability to measure in complete and exquisite detail the neuronal ``hardware'' that underlies specific behaviors, i.e. the map of how neurons connect with each other. This was previously difficult; however, significant advances in large volume serial electron microscopy (EM) has made this possible. EM is the gold standard for identifying and quantifying neuronal connections: with recent automation of ultra-thin sectioning of brains, fast EM imaging (e.g., gigahertz imaging rates), and machine learning algorithms for tracing neurons and connections comparable to human annotators, neuroscientists have produced datasets of neuronal connections with unprecedented detail. These datasets are publicly available, and are a promising avenue to test specific hypotheses about circuits, neuronal morphology, or the cellular composition of the neurons involved. Data about the cell biological level is critically relevant to behavior, but has not yet been incorporated into models that explain behavior -- in part because of limitations of traditional theory. 

